Scalene: Scripting-Language Aware Profiling for Python

Existing profilers for scripting languages (a.k.a. "glue" languages) like Python suffer from numerous problems that drastically limit their usefulness. They impose order-of-magnitude overheads, report information at too coarse a granularity, or fail in the face of threads. Worse, past profilers---essentially variants of their counterparts for C---are oblivious to the fact that optimizing code in scripting languages requires information about code spanning the divide between the scripting language and libraries written in compiled languages. This paper introduces scripting-language aware profiling, and presents Scalene, an implementation of scripting-language aware profiling for Python. Scalene employs a combination of sampling, inference, and disassembly of byte-codes to efficiently and precisely attribute execution time and memory usage to either Python, which developers can optimize, or library code, which they cannot. It includes a novel sampling memory allocator that reports line-level memory consumption and trends with low overhead, helping developers reduce footprints and identify leaks. Finally, it introduces a new metric, copy volume, to help developers root out insidious copying costs across the Python/library boundary, which can drastically degrade performance. Scalene works for single or multi-threaded Python code, is precise, reporting detailed information at the line granularity, while imposing modest overheads (26%--53%).

==> python.tex <==
While Python's features, such as its interactive read-eval-print loop,
make it relatively easy to use, a key contributor to its popularity is
its vast ecosystem of libraries. Python facilitates the integration of
libraries written in C, C++, or Java in the form of domain-specific
languages, leading to the proliferation of and popularity of systems
like the
\texttt{scikit-learn} machine learning toolkit and the \texttt{numpy} scientific
computing library.  This includes not only an extensive standard suite of
libraries but also systems for data science like Pandas and NumPy, and
machine learning platforms like OpenCV and Scikit-Learn.  It has
become especially popular for data science and machine learning: for
users of systems like Apache Spark and Google's TensorFlow, Python is
the primary interface.

% https://netflixtechblog.com/python-at-netflix-86b6028b3b3e



% https://github.com/apache/spark
% https://www.tensorflow.org/
% https://github.com/scikit-learn/scikit-learn

% Popular because of libraries



% Slow

\emph{Talk about versatility of Python here; maybe the \texttt{Decimal} example?}

These libraries are integrated into Python via bindings to other
languages like C++ or Java. This approach not only makes it easy to
port existing libraries to the Python platform, but also makes it
possible to overcome one of Python's major disadvantages: its
inefficiency.

Among popular programming languages, Python is one of the least
efficient, in both space and time. Python---in the form of its
standard CPython implementation---is a dynamically typed,
stack-machine based bytecode interpreter. In addition, all objects
are \emph{boxed}, prefaced with headers that contain at least type
information and reference counts. Boxed objects lead to increased
execution time (due to the need to repeatedly unbox and box objects),
degraded locality, and space overhead. For example, in Python 3 on a
64-bit system, a floating point number consumes 24 bytes,
an \texttt{int} consumes at least 28 bytes of memory, an empty string
(\texttt{""}) consumes 49 bytes, and an empty list consumes 64 bytes.


% Matrix multiplication example

In combination, these costs can be quite dramatic.

\texttt{Compare to NumPy}

However, Python falls short in both performance and
correctness. Thanks to its dynamic features, Python is slow, imposing
performance penalties as high as $60,000\times$ over optimized
low-level code (see Section~\ref{sec:perf}). It also imposes
substantial memory overhead: Python objects consume more than
$4\times$ as much memory as C/C++ objects, and its memory management
system can further multiply memory demands by as much as $32\times$.

Python imposes dramatic performance penalties compared to lower-level
languages. Consider the following example: a straightforward
implementation of matrix-matrix multiplication. Figure~\ref{fig:mmult} presents the
results of multiplying two $4K \times 4K$ matrices. This Python code re-
quires approximately 7 hours to run on a modern system. By contrast,
an optimized, parallel, vectorized C implementation takes just 0.41
seconds. In other words, pure Python code can impose an almost $60,000\times$
slowdown. Worse, this gap seems insurmountable using conventional
compiler technology. For example, running the above code with PyPy, a
modern JIT compiler for Python dramatically increases its performance:
it runs roughly 20$\times$ faster. While this is impressive (though, in our
experience, atypical), it still performs 3000$\times$ slower than optimized
low-level code.

Besides being slow, Python is extremely memory inefficient. To
illustrate: an integer---normally 4 or 8 bytes in C code---consumes at
least 24 bytes in Python. Similarly, an empty list consumes 64 bytes,
a string with just one character requires 50 bytes, and an empty
dictionary consumes 240 bytes. Python's memory inefficiency degrades
performance by severely reducing the effectiveness of hardware caches,
which hold far less useful data than when running low-level code (in
the worst case, leading to paging). In the matrix multiplication
example, the Python version requires 1.5GB of memory, while a
corresponding C program uses just 192MB. This increased memory demand
effectively forces Python programs to use far less data than programs
written in other languages. The only alternative is for developers to
rewrite the code to use external libraries.

\begin{myverbbox}[\small]{\mmult}
for i in range(n):
  for j in range(n):
    for k in range(n): 
      C[i][j] += A[i][k] * B[k][j]
\end{myverbbox}

%\begin{figure}[!t]
%  \centering
%  \mmult
%\end{figure*}

\begin{figure}[!t]
  \centering
  \begin{subfigure}[t]{3in}
    \centering
    \mmult
%    \vspace{2em}
  \end{subfigure}
  \begin{subfigure}[t]{3in}
    \centering
    \includegraphics[width=3in]{mmult-graph-small}
    \vspace{1em}
  \end{subfigure}
  \caption{Python matrix-matrix multiplication and its overhead versus
    optimized low-level code (Leiserson et al., from Hennessy and Patterson's
    Turing Lecture).\label{fig:mm-graph} }
\end{figure}



